Energy-Constrained Active Exploration Under Incremental-Resolution Symbolic Perception

In this work, we consider the problem of autonomous exploration in search of targets while respecting a fixed energy budget. The robot is equipped with an incremental-resolution symbolic perception module wherein the perception of targets in the environment improves as the robot's distance from targets decreases. We assume no prior information about the total number of targets, their locations as well as their possible distribution within the environment. This work proposes a novel decision-making framework for the resulting constrained sequential decision-making problem by first converting it into a reward maximization problem on a product graph computed offline. It is then solved online as a Mixed-Integer Linear Program (MILP) where the knowledge about the environment is updated at each step, combining automata-based and MILP-based techniques. We demonstrate the efficacy of our approach with the help of a case study and present empirical evaluation in terms of expected regret. Furthermore, the runtime performance shows that online planning can be efficiently performed for moderately-sized grid environments.

==> problem.tex <==
% \clearpage
\section{Problem Setup}
\label{sec:problem}
Consider a planar grid environment with objects of interest (e.g., artifacts and victims),
referred to as \textbf{\textit{targets}}, see Fig.~\ref{fig:grid_perception}.
These targets are hidden in the environment and \cdc{no prior information about  the total number of targets, their locations or the frequencies of their occurrences is available.}
   % Consider a planar environment with hidden targets.
Given an autonomous robot moving through this environment 
  % the robot motion model\sofie{[Perhaps first state that we have a robot moving around that wants to collect these targets. Afterward, you can make it more precise.]} and 
with a \cdc{\textbf{fixed energy budget}}, our objective is to design a path that services as many of these targets as possible and ultimately reaches the given \cdc{\textbf{goal location}}. 
In the following, we describe various components of the problem. 


% We will use the help of an example and we will follow up with a formal definition of the problem \st{of }\sofie{the}\st{ energy-constrained exploration with incremental-resolution symbolic perception. }\sofie{\itshape Consider for now removing incremental-resolution symbolic perception or  introduce it in words. Now it is still undefined and could confuse people.}


\noindent %\subsection{\
\textbf{Robot Motion and Environment}
Let $X$ denote the set of locations, i.e., grid cells.
\cdc{The robot is able to move \textit{North, East, South, West} to adjacent locations  in a deterministic manner}.
The initial location $x_{init}$ of the robot \cdc{and the goal location $x_{goal}$ are} given.

% The robot is tasked with finding and servicing as many targets as possible while moving towards a goal location $x_{goal}$.
Let the set of \emph{targets} be denoted by $\mathcal{L}$.
Each location may contain a single target, another object of no interest to the robot or nothing at all.
We associate each cell with a \textit{ground truth symbol} from a given set $\Pi$ that includes the targets,
$\mathcal{L} \subseteq \Pi$.
The symbols in $\Pi$ contain full semantic information about targets and objects.
% \disha{$\Pi$ comprises of all symbols in the environment that cannot be further refined. }
% If a cell contains the target $\ell \in \mathcal{L}$ then its ground truth symbol is $\ell$.
% symbols in $\Pi \setminus \mathcal{L}$ capture objects of no interest to the mission and absence of any object or target.
% The \textit{ground truth symbol} of a cell containing target $\ell \in \mathcal{L}$ if a target is present or
% ${\bowtie}$ if there is no target.
% The set of ground truth symbols is $\Pi = \mathcal{L} \cup \{{\bowtie}\}$, and is known a priori.
A cell that does not contain targets or objects is called \textit{\empty{empty}} and is associated with the symbol $\ell_\emptyset \in \Pi$.
We assume that the environment is static.
Furthermore, the ground truth symbols are independent between locations.
Thus, the knowledge about one cell does not provide more information about any other cell.


% \begin{assumption}
% \label{assump:preserve} Each grid cell may have at most one ground-truth symbol $l\in \Pi$. 
% \end{assumption}


\begin{figure}[t]
\centering
    \includegraphics[width=\columnwidth]{images/grid_refinement_final.png}    
    % \begin{subfigure}[h]{.32\linewidth}
    %     \centering
    % 	\includegraphics[width=\linewidth]{images/t2.png}
    % \caption{}
    % \end{subfigure}
    \caption{\small{(a) A robot with sensing range limited to its immediate neighbors (blue colored cells). Thus, the robot has no observations about all grey colored cells. (b) shows an instance of refinement in symbolic perception where the \textit{root} corresponds to no observation being available and for each subsequent layer, the symbols are refined. Thus, (a) and (b) depict the metric and symbolic representation of the agent's perception, respectively. As the robot moves along the green arrow, its observation about cell $x_1$ changes from $\mathrm{Fire}$ to $\mathrm{Class\_A\_Fire}$ with probability $p6$.}} \label{fig:grid_perception}
\end{figure}

\begin{example}
\label{ex:labels}
Consider the robot in the $4\times4$ grid environment in Fig.~\ref{fig:grid_perception}(a) containing fire and victim targets.
% Figure~\ref{fig:grid_perception} shows an example of a 4 by 4 grid environment.
% The robot can deterministically move can move \textit{North, East, South, West}.
% This implies that we can represent the environment as a square grid for which we know the coordinates of each grid cell.}
% The initial location (cell) of the robot given, and it is tasked with reaching the given goal location.
% Consider an autonomous robot navigating a planar, square-grid environment where targets may be present as shown in Fig.~\ref{fig:grid_perception}(a).
% The geometric coordinates of each grid-cell are known and the robot can move \textit{Up, Down, Left, Right} deterministically from the current location.
The robot is tasked to satisfy as many instances of rescuing severely injured victims and extinguishing Class-A fire as possible, if they are present, and reach the goal location.
% The \textit{ground truth symbol} of a cell is a symbol that corresponds to the object present at that particular cell. We denote the set of ground truth symbols as $\Pi$. These symbols of the grid are \textit{a priori} unknown. The \textit{targets} (objects of interest) are denoted by $\mathcal{L}$, $\mathcal{L} \subseteq \Pi$.
The set of symbols is $\mathcal{I}_0 = \{\mathrm{Severely\_Injured\_Victim}, \linebreak \mathrm{Mildly\_Injured\_Victim}, \mathrm{Class\_A\_Fire}, \mathrm{Class\_B\_Fire}, \linebreak \mathrm{Other}\}$; $\mathcal{L} = \{\mathrm{Severely\_Injured\_Victim}, \mathrm{Class\_A\_Fire}\}$.
% We assume that a set of all potential symbols $\Pi$ is given and a symbol at a particular grid cell does not change over time, i.e., the environment is static. Furthermore, the ground truth symbols are independent and each grid cell may have at most one ground truth symbol.
\end{example}

In this paper, we focus on the discrete (high-level) motion of the robot in the grid environment. We assume that there are low-level controllers to enforce the motion of the robots between cells and staying at a cell~\cite{lindemann2009simple}.

% \textcolor{pink}{[Note that in the next section you will talk about both continuous control and discrete control. It could be good to lightly talk about it here too. Something like although the robots final controller will implement a continuous motion, we can do its planning first over a discrete space. That is, ....]}

\subsection{ Energy Constraints and \cdc{Target rewards}}

\indent The robot has a fixed energy budget $\mathbf{E}$ that implicitly bounds the horizon over which the exploration mission can be performed.
% Each transition between adjacent grid cells costs a unit of energy $e_m$.
% \cristi{
Each transition between adjacent grid cells $x, x' \in X$ takes $w(x, x') > 0$ energy to perform.
% [ignore for now.]}
% \sofie{[\itshape Does $e_m$ have to be constant or can it be a function of the cell pair?]}

A target in the environment is \emph{satisfied} when the robot moves to a cell containing that target,
and collects a \emph{target reward} $\mathbf{r}(\ell)$, $\ell \in \mathcal{L}$. \disha{The rewards may capture priorities over targets}. 
The energy required for servicing each symbol is captured by the map $\mathbf{e}: \Pi \to \mathbb{Z}_{\geq 0}$.
For all \emph{targets} $\ell \in \mathcal{L}$ the servicing energy $\textbf{e}(\ell) > 0$, while for any other symbol $\textbf{e}(\ell) = 0$, $\forall \ell \in \Pi \setminus \mathcal{L}$.
% The set of energy values required to satisfy each type of target is given and denoted by $\{\mathbf{E}_\ell\}_{\ell \in \mathcal{L}}$.


\subsection{Incremental-resolution Perception}
\label{sec:incremental-perception}
% - incremental symbols 
% - Ground truth symbols correctly observed only for the current cell - Some symbols can be observed for the cells within the sensing range of the robot in addition to the ground truth symbols - these are referred to as the incrememntal symbols. 

% Distances  
% resolution levels 
% Refinement; descendents 


% intro to perception - 
The robot is equipped with a perception module necessary for detecting the potential targets. 
We consider sensing within a limited range around the robot that provides observations with
\emph{symbolic resolution} decreasing with the distance from the robot.
% To emulate real-world limitations, the sensing range is considered to be limited up to a few cells in the vicinity of the robot location.
The sensing range $D \in \mathbb{N}$ allows the robot to observe all cells $x'$ within
$D$-Manhattan distance away from the current cell $x$, i.e., $||x - x'||_1 \leq D$ for all $x' \in X$. 
\footnote{
With a slight abuse of notation, we identify a cell $x$ with its integer coordinates in the grid.}.
We denote by $\mathcal{N}_x^d$ all cells $x'$ for which $\vert \vert x' - x \vert\vert = d$,
where $x$ is the current robot location and $d\in \mathbb{Z}_{\geq0}$. Thus, the set of visible cells is $\mathcal{N}_x^{\leq D} = \mathcal{N}_x^0 \cup \ldots \cup \mathcal{N}_x^D$.



% obs - distance rel; neighbors def - link it to depth 
The symbolic perception information is modeled in an incremental-resolution manner as described in \cite{kamale2022cautious}. As the robot moves through the environment, it deterministically observes the symbols of cells within the sensing range $D$ at different resolution levels depending on its distance from them.
For each distance $d \in \mathbb{Z}_\geq 0$, we associate a set of symbols $\mathcal{I}_d$
that can be observed at the Manhattan distance $d$ by the robot.
The set of all symbols is denoted by $\mathcal{I} = \bigcup_{d=0}^D \mathcal{I}_d$.
At its current location, the robot can observe only ground truth symbols, i.e., $\mathcal{I}_0 \subseteq \Pi$.
Some ground truth symbols may be observed from farther away ($d\geq 1$), see Fig.~\ref{fig:grid_perception}.
The symbols $\mathcal{I} \setminus \Pi$ are called \emph{incremental symbols} and capture lower resolution (incomplete) semantic information.

Moreover, we are given a priori distribution on what symbols may be observed by moving one cell closer to an observed cell $x'$.
Formally, for any $\ell \in \mathcal{I}_d$ the prior probability distribution $p_\ell: \mathcal{I}_{d-1} \to [0, 1]$ is given, where $p_\ell(\ell') > 0$ iff the symbol $\ell'$ can be observed for cell $x'$ at distance $d-1$ given that at distance $d$ symbol $\ell$ was observed.
For distance $d \geq D+1$, no observations are available.
For uniformity of presentation, we associate this mode with a \emph{root} symbol $\ell_{\bowtie}$ and prior $p_{\ell_{\bowtie}} : \mathcal{I}_D \to [0, 1]$, where $p_{\ell_{\bowtie}}(\ell) > 0$ for all $\ell \in \mathcal{I}_D$.
The relationship captured by priors $\left\{p_\ell\right\}_{\ell \in \mathcal{I} \cup \{\ell_{\bowtie}\}}$ represents the symbolic \emph{perception refinement} structure of the robot's sensing. 

\iffalse
\disha{\sout{
% \cristi{For example, a vision-based perception system may be able to ... [Also cite your ICRA paper here without describing the content]}
% \sofie{\itshape Do you want to bring this in as a specific "sensor"? It could be easier to justify if you state that as in [1], we assume that the perception information can be modeled in an incremental fashion. More precisely, as depicted in ...}
In this model, the ground truth symbols $l \in \Pi$ are observed only for the current robot location.
For neighboring cells within the sensing range, some partial symbolic information, referred to as \textit{incremental symbols}, can be observed.
% We refer to this partial symbolic information as \textit{incremental symbols}.
The set of all possible incremental symbols is $\mathcal{I}$.
% Naturally, no symbols are observed for cells beyond the sensing range $d$. %, and includes ground truth symbol, $\Pi\subset \mathcal{I}$.
As the robot physically moves closer to a cell containing a target, its observation about the target cell sequentially progresses through a series of incremental symbols and finally reaches a unique ground truth symbol as the robot transitions into the cell containing the target.
}

\sout{
The relationship between incremental and ground truth symbols is given. We refer to this symbolic relationship as \textit{perception refinement} represented as a DAG $\Lambda_\Delta = (\vee_\Delta, E_\Delta)$ where $\vee_\Delta = \Pi \cup \mathcal{I}$ and $E_\Delta = (l,l', p_{l,l'})$ where $p_{l,l'} \in [0,1]$ represents the probability with which the observed incremental symbol $l$ actually leads to a incremental/ ground truth symbol $l'$. Thus, $l'$ is a direct descendent of $l$ if $p_{l',l}$ is non-zero. We assume that these probabilities are given and remain fixed throughout the mission. 
}

\begin{definition}[Resolution-level]
\sout{
 For a given perception refinement, the resolution-level of symbol $l, l \in \vee_\Delta$ is defined as the maximum number of edges between the root of the refinement and the node $l$, and is denoted as $\rho(l)$.
 }
\end{definition}
}

\disha{\sout{
% We represent the incremental symbols as a directed acyclic graph (DAG) to (a) capture the refinement of symbolic information about cells, and (b) to highlight the cumulative nature of the perception process.
% For the latter, we assume that robot's (partial) information about a cell is persistent, i.e., the cell's symbol may only be refined when the robot moved closer to it.
% % This also implies that there is no information gain about the cell until robot moves closer to it.
% Thus, the tree models knowledge about cells and not just observations, where the root of the tree denotes that no observation is available.
% We refer the reader to \cite{kamale2022cautious} for a detailed discussion on incremental-resolution symbolic perception.


% \disha{In addition to the hierarchical structure of the symbolic perception system,
% we assume that a prior distribution of symbol refinement is given.
% Let $M = \mathcal{L} \cup \mathcal{I}$.
% For each $m, m' \in M$, $p_{m,m'} > 0$ captures the probability that
% symbol $m$ is actually symbol $m'$ when $m'$ is a direct descendent of $m$ in
% the perception tree (i.e., the robot moves one cell closer),
% $p_{m,m} = 1$ (i.e., the robot does not move or moves away),
% and $p_{m,m'} = 0$ otherwise. \disha{Henceforth, this perception structure is referred to as \textit{perception refinement}. }

For a given sensing range $D$, the maximum possible resolution is $\rho_{max} = D+1$. 
}}
\fi

\begin{example}[Continuation of Ex.~\ref{ex:labels}]
Fig.~\ref{fig:grid_perception}(b) is an instance of perception refinement with $D=1$. The directed edges indicate the evolution of symbolic information.
The robot can observe the ground truth symbols $\mathcal{I}_0$ for its current location and the incremental symbols $\mathcal{I}_1 = \{\mathrm{Victim}, \mathrm{Fire}, \mathrm{Other}\}$ for the cells that are one-step away.
The \textit{root} symbol ${\ell_{\bowtie}}$ corresponds to no observation available and that is the current robot observation for cells beyond sensing range.
Thus, the (a) and (b) denote the metric and symbolic representation of the perception model.
% \cristi{Note that, the refinement depends on the sensing depth of the robot and may not be unique. [What do you mean?]}
\end{example}


% \begin{assumption}
% \label{assump:accumulation}The resolution level contains new symbolic information in addition to all the accumulated information up to the previous layer. 
% \end{assumption}
 
% \sofie{[\itshape it could be good to differentiate between observation and knowledge.
% A cell with root value, is a cell about which you do not have knowledge about.
% If you get within a specific sensing range you receive ... ]}

% \begin{figure}[h]
%     \centering
%     \includegraphics[scale=0.4]{images/motiv_warehouse.png}
%     \caption{An aerial robot with limited energy budget is tasked with locating a warehouse with the given description in a large environment.}
%     \label{fig:warehouse}
% \end{figure}

% \disha{For each $m, m' \in M$, $p_{m,m'} > 0$ captures the probability that if a particular cell }

% \sofie{[\itshape I think we can formulate this a bit stronger. Let me think about how.]}
% In this work, the perception symbol changes probabilistically, with a known distribution, as the robot physically moves closer to the event. Each state also contains a self-loop with probability one indicating that no further information was obtained regarding that object. These self-loops have been omitted for brevity. 

% \textit{Remark:} 
%  We assume that the perception state, which defines the information obtained via perception, is persistent. That is the perception state of the cell is preserved even when the robot continues to stay at its current location or moves away from the cell containing the event. Moreover, for a given setting, the perception refinement model (states, transitions, and transition probabilities) is assumed to be invariant throughout the course of the mission. 


With this, the problem of energy-constrained active exploration is defined as follows: 

\begin{problem}[Energy-Constrained Active Exploration]
\label{prob:active_decision}
Given a robot with incremental-resolution symbolic perception refinement $\left\{p_\ell\right\}_{\ell \in \mathcal{I} \cup \{\ell_{\bowtie}\}}$,
the energy budget $\mathbf{E}$
deployed in a grid environment with unknown cell symbols, and the set of ground truth symbols $\mathcal{L}$
with servicing rewards $\mathbf{r}$ and energy costs $\mathbf{e}$,
find a path such that the robot maximizes the sum of target servicing rewards
and reaches the goal location $x_{goal}$
while respecting the energy budget.
% Given a robot with incremental-resolution symbolic perception refinement $\Lambda_\Delta$, the energy budget $\mathbf{E}$
% deployed in a grid environment with unknown cell symbols, and the set of ground truth symbols $\mathcal{L}$
% with servicing energy costs $\{\mathbf{E_\ell}\}_{\ell \in \mathcal{L}}$,
% % and the relationship between the incremental and ground truth symbols,
% find a path such that the robot satisfies as many targets as possible and reaches the goal location $x_{goal}$
% while respecting the energy budget.
\end{problem}


\iffalse
\subsection{Toy Example}



We describe Problem~\ref{prob:active_decision} with the help of the following example. As shown in Fig.~\ref{fig:grid_perception}, a robot is tasked to satisfy as many occurrences of the targets $\mathcal{L} = \{Class\_A\_Fire, Severely\_injured\_Victim\}$ as possible. The robot can observe the ground truth symbol of its current cell and the incremental symbols of the cells that are one-step away from its current location. An ideal strategy would be to design a path that allows to robot to collect at least ''partially see" all the cells of the environment. However, this strategy is infeasible in resource-constrained scenarios. 

If the robot chooses to follow the path shown using green arrow, the

% As compared to our previous work, we extend the notion of incremental symbolic perception such that the state transitions are stochastic (modeled as probability distributions). 
Fig.~\ref{fig:grid_perception} depicts a multi-resolution perception model for a search-and-rescue scenario. An autonomous ground robot with limited energy budget is deployed to satisfy the targets of rescuing severely injured and mildly injured victims and extinguish fire, if any and reach the goal location. The ground truth event \textit{fire\textsubscript{A}} is located at cell 5. We assume a sensing range of 1 cell i.e., the robot can sense some information about each cell that is within two cells away from the current robot location. These cells are shown in light grey, light blue and blue with the robot present at cell 0. The cells outside the sensing range of the robot are shown in white and for all such cells, the robot perception corresponds to \textit{''Root"} in Fig.~\ref{subfig:perception_refinement}.   

 

 For each grid cell, the robot is in exactly one of the states of the perception refinement as follows: With robot at cell 0, for each cell 2-steps away, it perceives whether an event is present (cell 5) or not (cells 6-12). For each cell one-step away (cells 1-4), the robot knows the type of event present, if any. Following the green path, as the robot moves one cell closer to cell 5, its knowledge about the event at cell 5 improves further that it is \textit{Fire}. Finally, when the robot moves to the cell 5, it exactly knows the ground truth event. If the robot were to instead take the brown path, the most knowledge the robot has about cell 5 is the symbol \textit{Fire} and since the environment is static, this symbol persists. In other words, the history of observation is preserved. For conciseness, we do not show the self-loops in the perception refinement. 


\fi
 
% \noindent \textbf{Robot Perception Model as MDP}

% \begin{figure}
%     \centering
%     \includegraphics[width = \linewidth]{images/grid_perception.png}
%     \caption{The colored regions show the cells of the environment within the sensing range of the robot. The level of information it knows about neighbors is color-coded in the adjacent refinement MDP. }
%     \label{fig:grid_percept}
% \end{figure}





% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\columnwidth]{images/simple_refinement.png}
%     \caption{Caption}
%     \label{fig:refinement}
% \end{figure}

% Fig.~\ref{fig:warehouse} shows an example perception refinement model $\mathcal{M}$. The root node of $\mathcal{M}$ denotes a symbolic sensor input and each subsequent layer denotes a finer symbolic detail captured as the robot physically moves closer to an object / event. The terminal nodes correspond to the symbolic events identified as a whole. The black arrows depict transitions corresponding to action $``move"$ and the blue arrows correspond to the action $``stay"$. Wherever not shown, the transition probabilities are one. 






==> solution.tex <==
% \subsection{Energy budget allocation}





